Detecting Pretraining Data from Large Language Models

Although large language models (LLMs) are widely deployed, the data used to train them is rarely disclosed. Given the incredible scale of this data, up to trillions of tokens, it is all but certain that it includes potentially problematic text such as copyrighted materials, personally identifiable information, and test data for widely reported reference benchmarks. However, we currently have no way to know which data of these types is included or in what proportions. In this paper, we study the pretraining data detection problem: given a piece of text and black-box access to an LLM without knowing the pretraining data, can we determine if the model was trained on the provided text? To facilitate this study, we introduce a dynamic benchmark WIKIMIA that uses data created before and after model training to support gold truth detection. We also introduce a new detection method Min-K% Prob based on a simple hypothesis: an unseen example is likely to contain a few outlier words with low probabilities under the LLM, while a seen example is less likely to have words with such low probabilities. Min-K% Prob can be applied without any knowledge about the pretraining corpus or any additional training, departing from previous detection methods that require training a reference model on data that is similar to the pretraining data. Moreover, our experiments demonstrate that Min-K% Prob achieves a 7.4% improvement on WIKIMIA over these previous methods. We apply Min-K% Prob to three real-world scenarios, copyrighted book detection, contaminated downstream example detection and privacy auditing of machine unlearning, and find it a consistently effective solution.

==> section/analysis.tex <==
r

==> table/downstream_multiplicity.tex <==
\begin{table*}[h]
\centering
\footnotesize
\begin{tabular}{ccccccc}
\toprule
\textbf{multiplicity} & \textbf{BoolQ} & \textbf{Commonsense} & \textbf{Dyck language} & \textbf{IMDB} & \textbf{LSAT QA} & \textbf{Truthful QA} \\
\midrule
\multicolumn{7}{c}{\GD{\textbf{\model}}} \\
1 & 0.912 & 0.939 & 0.602 & 0.975 & 0.766 & 0.925\\
2 & 0.976 & 0.995 & 0.607 & 1.000 & 0.852 & 0.953\\
3 & 1.000 & 0.999 & 0.594 & 1.000 & 0.969 & 1.000\\
4 & 0.989 & 1.000 & 0.608 & 1.000 & 0.983 & 1.000\\
5+ & 0.997 & 1.000 & 0.610 & 1.000 & 0.992 & 1.000\\
\bottomrule
%

\end{tabular}
\caption{AUC scores for detecting contaminant downstream examples using reference-based and reference-free methods. \textbf{Bold} shows the best reference-free AUC within each column. ~\mz{Please consider turning this table into a graph as well and only show min-k prob. }}
\end{table*}




==> table/downstream_scaling_news_august.tex <==
\begin{table*}[h]
\centering
\footnotesize
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \textbf{1000} & \textbf{5000} & \textbf{10000} \\
\midrule
PPL & 0.635 & 0.562 & 0.526 \\
\model & 0.633 & 0.562 & 0.530 \\
\bottomrule
%

\end{tabular}
\caption{AUC scores for detecting contaminant examples from News August 2023 using perplexity and \model at different corpus sizes. \mz{consider tunring this table into a graph, see comment above.}}
\end{table*}




==> table/downstream_scaling_tasks.tex <==
\newcommand{\GD}[1]{\cellcolor{gray!15} \text{{#1}}}

\begin{table*}[h]
\centering
\footnotesize
\begin{tabular}{rcccccc}
\toprule
\textbf{Rate (\%)} & \textbf{BoolQ} & \textbf{Commonsense QA} & \textbf{Dyck} & \textbf{IMDB} & \textbf{LSAT QA} & \textbf{Truthful QA} \\
\midrule
\multicolumn{7}{c}{\GD{\textbf{\model}}} \\
0.1 & 0.958 & 0.977 & 0.597 & 0.985 & 0.892 & 0.938 \\
1.0 & 0.954 & 0.962 & 0.515 & 0.971 & 0.871 & 0.944 \\
100.0 & 0.722 & 0.639 & 0.539 & 0.794 & 0.659 & 0.628 \\
\bottomrule
%

\end{tabular}
\caption{AUC scores for detecting contaminant downstream examples using perplexity and \model at different data contamination rates. \mz{let's add 10 percent and let's turn this table and table 4 into two side-by-side graphs, where x axis is the contamination rate and the y axis is the score. You can consider present average AUCs? Also we only need to show min-k prob.}}
\end{table*}




==> table/main_complete_results.tex <==



\newcommand{\SD}[1]{\cellcolor{green!15} \text{{#1}}}
\newcommand{\ID}[1]{\cellcolor{yellow!35} \text{{#1}}}




\begin{table*}[ht]
\centering
\footnotesize
\begin{tabular}{lccccccccccc}
\toprule
& \multicolumn{2}{c}{\textbf{Pythia-2.8B}} & \multicolumn{2}{c}{\textbf{NeoX-20B}} & \multicolumn{2}{c}{\textbf{LLaMA-30B}} & \multicolumn{2}{c}{\textbf{LLaMA-65B}} & \multicolumn{2}{c}{\textbf{OPT-66B}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
\textbf{Method} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textit{Ori.} & \textit{Para.} & \textbf{Avg.} \\
\midrule
\multicolumn{3}{l}{\SD{\textit{\textbf{Reference based: Calibrate to}}}} & & & & & & & & & \\
Pythia-70M & 0.60 & 0.58 & 0.69 & 0.67 & 0.67 & 0.63 & 0.68 & 0.65 & 0.63 & 0.60 & 0.64 \\
Neo-125M & 0.57 & 0.53 & 0.68 & 0.65 & 0.65 & 0.60 & 0.66 & 0.62 & 0.61 & 0.57 & 0.61 \\
OPT-350M & 0.63 & 0.61 & 0.73 & 0.71 & 0.69 & 0.65 & 0.70 & 0.66 & 0.67 & 0.64 & 0.67 \\
LLaMA-7B & 0.44 & 0.43 & 0.68 & 0.64 & 0.72 & 0.64 & \textbf{0.74} & 0.70 & 0.52 & 0.48 & 0.60 \\
\midrule
\multicolumn{1}{l}{\textit{\ID{\textbf{Reference free}}}} & & & & & & & & & & & \\
Neighbor & 0.61 & 0.59 & 0.68 & 0.58 & 0.71 & 0.62 & 0.71 & 0.69 & 0.65 & 0.62 & 0.65 \\
PPL & 0.61 & 0.61 & 0.70 & 0.70 & 0.70 & 0.70 & 0.71 & 0.72 & 0.66 & 0.64 & 0.67 \\
Zlib & 0.65 & 0.54 & 0.72 & 0.62 & 0.72 & 0.64 & 0.72 & 0.66 & 0.67 & 0.57 & 0.65 \\
Lowercase & 0.59 & 0.60 & 0.68 & 0.67 & 0.59 & 0.54 & 0.63 & 0.60 & 0.59 & 0.58 & 0.61 \\
\model & \textbf{0.67} & \textbf{0.66} & \textbf{0.76} & \textbf{0.74} & \textbf{0.74} & \textbf{0.73} & \textbf{0.74} & \textbf{0.74} & \textbf{0.71} & \textbf{0.69} & \textbf{0.72} \\
\bottomrule
%

\end{tabular}
\caption{AUC score for detecting pretraining examples from the given model on \data for \model and baseline reference-based and reference-free methods. \textit{Ori.} and \textit{Para.} denote the original and paraphrase settings, respectively. \textbf{Bold} shows the best AUC within each column. \weijia{mention why reference-based is worse than reference-free method. only keep the smaller model...}} \label{tab:main}
\end{table*}

